Misspecified Cram\'er-Rao Bound of RIS-aided Localization under Geometry Mismatch

In 5G/6G wireless systems, reconfigurable intelligent surfaces (RIS) can play a role as a passive anchor to enable and enhance localization in various scenarios. However, most existing RIS-aided localization works assume that the geometry of the RIS is perfectly known, which is not realistic in practice due to calibration errors. In this work, we derive the misspecified Cram\'er-Rao bound (MCRB) for a single-input-single-output RIS-aided localization system with RIS geometry mismatch. Specifically, unlike most existing works that use numerical methods, we propose a closed-form solution to the pseudo-true parameter determination problem for MCRB analysis. Simulation results demonstrate the validity of the derived pseudo-true parameters and MCRB, and show that the RIS geometry mismatch causes performance saturation in the high signal-to-noise ratio regions.

==> RIS Geometry Mismatch/Acronyms.tex <==
% \newlist{acronyms}{description}{1}
% \setlist[acronyms]{
% labelwidth = 4.5em,
% leftmargin = 5em,
% noitemsep,
% itemindent = 0pt}
% \DeclareAcroListStyle{mystyle}{list}{ list = acronyms }
% \acsetup{ list-style = mystyle }

\DeclareAcronym{5g}{
short=5G,
long= fifth generation,
}
\DeclareAcronym{6g}{
short=6G,
long= sixth generation,
}
\DeclareAcronym{3d}{
short=3D,
long= three-dimensional,
}
\DeclareAcronym{2d}{
short=2D,
long= two-dimensional,
}
\DeclareAcronym{1d}{
short=1D,
long= one-dimensional,
}
\DeclareAcronym{aod}{
short=AOD,
long= angle-of-departure,
}
\DeclareAcronym{aosa}{
short=AOSA,
long= array-of-subarray,
}
\DeclareAcronym{adod}{
short=ADOD,
long= angle-difference-of-departure,
}
\DeclareAcronym{aoa}{
short=AOA,
long= angle-of-arrival,
}
\DeclareAcronym{adc}{
short=ADC,
long= analog to digital converter,
}
\DeclareAcronym{aeb}{
short=AEB,
long= angle error bound,
}
\DeclareAcronym{av}{
short=AV,
long= autonomous vehicle,
}
\DeclareAcronym{bs}{
short=BS,
long= base station,
}

\DeclareAcronym{csi}{
short=CSI,
long= channel state information,
}
\DeclareAcronym{cfo}{
short=CFO,
long= carrier frequency offset,
}
\DeclareAcronym{ceb}{
short=CEB,
long= clock error bound,
}
\DeclareAcronym{coa}{
short=COA,
long= curvature-of-arrival,
}
\DeclareAcronym{crb}{
short=CRB,
long= Cram\'er-Rao bound,
}
\DeclareAcronym{ccrb}{
short=CCRB,
long= constrained Cram\'er-Rao bound,
}
\DeclareAcronym{cmos}{
short=CMOS,
long= complementary metal-oxide-semiconductor,
}
\DeclareAcronym{crlb}{
short=CRLB,
long= Cram\'er-Rao lower bound,
}
\DeclareAcronym{cdf}{
short=CDF,
long= cumulative distribution function,
}
\DeclareAcronym{cp}{
short=CP,
long= cyclic prefix,
}
\DeclareAcronym{dac}{
short=DAC,
long= digital to analog converter,
}
\DeclareAcronym{dfl}{
short=DFL,
long= device-free localization,
}
\DeclareAcronym{dmimo}{
short=D-MIMO,
long= distributed MIMO,
}
\DeclareAcronym{dlprs}{
short=DL-PRS,
long= downlink positioning reference signal,
}
\DeclareAcronym{d2d}{
short=D2D,
long= device-to-device,
}
\DeclareAcronym{dftsofdm}{
short=DFT-s-OFDM,
long= discrete-Fourier-transform spread OFDM,
}
\DeclareAcronym{dl}{
short=DL,
long= deep learning,
}
\DeclareAcronym{gps}{
short=GPS,
long= global positioning system,
}
\DeclareAcronym{gnss}{
short=GNSS,
long= global navigation satellite system,
}
\DeclareAcronym{fim}{
short=FIM,
long = Fisher information matrix,
}
\DeclareAcronym{hwi}{
short=HWI,
long= hardware impairment,
}
\DeclareAcronym{hemt}{
short=HEMT,
long= high electron mobility transistor,
}
\DeclareAcronym{hbt}{
short=HBT,
long= heterojunction bipolar transistors,
}
\DeclareAcronym{iot}{
short=IoT,
long= internet of things,
}
\DeclareAcronym{imu}{
short=IMU,
long= inertial measurement unit,
}
\DeclareAcronym{isac}{
short=ISAC,
long= integrated sensing and communication,
}
\DeclareAcronym{iqi}{
short=IQI,
long= in-phase and quadrature imbalance,
}
\DeclareAcronym{ip}{
short=IP,
long= incidence point,
}
\DeclareAcronym{ia}{
short=IA,
long= initial access,
}
\DeclareAcronym{kpi}{
short=KPI,
long= key performance indicator,
}
\DeclareAcronym{kf}{
short=KF,
long= Kalman filter,
}
\DeclareAcronym{ekf}{
short=EKF,
long= extended Kalman filter,
}
\DeclareAcronym{ukf}{
short=UKF,
long= unscented Kalman filter,
}
\DeclareAcronym{ckf}{
short=CKF,
long= cubature Kalman filter,
}
\DeclareAcronym{pf}{
short=PF,
long= particle filter,
}
\DeclareAcronym{lb}{
short=LB,
long= lower bound,
}
\DeclareAcronym{lse}{
short=LSE,
long= least-square estimation,
}
\DeclareAcronym{ls}{
short=LS,
long= least-squares,
}
\DeclareAcronym{lo}{
short=LO,
long= local oscillator,
}
\DeclareAcronym{los}{
short=LOS,
long= line-of-sight,
}
\DeclareAcronym{mc}{
short=MC,
long= mutual coupling,
}
\DeclareAcronym{mac}{
short=MAC,
long= medium access control,
}
\DeclareAcronym{meb}{
short=MEB,
long= mapping error bound,
}
\DeclareAcronym{mcrb}{
short=MCRB,
long= misspecified Cram\'er-Rao bound,
}
\DeclareAcronym{mds}{
short=MDS,
long= multidimensional scaling ,
}
\DeclareAcronym{mimo}{
short=MIMO,
long= multiple-input-multiple-output,
}
\DeclareAcronym{siso}{
short=SISO,
long= single-input-single-output,
}
\DeclareAcronym{mm}{
short=MM,
long= mismatched model,
}
\DeclareAcronym{mpc}{
short=MPC,
long= multipath components,
}
\DeclareAcronym{mmwave}{
short=mmWave,
long= millimeter wave,
}
\DeclareAcronym{mmle}{
short=MMLE,
long= mismatched maximum likelihood estimation,
}
\DeclareAcronym{mems}{
short=MEMS,
long= micro-electro-mechanical system,
}
\DeclareAcronym{mle}{
short=MLE,
long= maximum likelihood estimation,
}
\DeclareAcronym{ml}{
short=ML,
long= maximum likelihood,
}
\DeclareAcronym{nlos}{
short=NLOS,
long= none-line-of-sight,
}
\DeclareAcronym{ofdm}{
short=OFDM,
long= orthogonal frequency-division multiplexing,
}
\DeclareAcronym{oeb}{
short=OEB,
long= orientation error bound,
}
\DeclareAcronym{otfs}{
short=OTFS,
long= orthogonal time-frequency space,
}
\DeclareAcronym{pdf}{
short=PDF,
long= probability density function,
}
\DeclareAcronym{papr}{
short=PAPR,
long= peak-to-average-power ratio,
}
\DeclareAcronym{pan}{
short=PAN,
long= power amplifier nonlinearity,
}
\DeclareAcronym{pa}{
short=PA,
long= power amplifier,
}
\DeclareAcronym{ps}{
short=PS,
long= phase shifter,
}
\DeclareAcronym{pn}{
short=PN,
long= phase noise,
}
\DeclareAcronym{poa}{
short=POA,
long= phase-of-arrival,
}
\DeclareAcronym{pwm}{
short=PWM,
long= planar wave model,
}
\DeclareAcronym{pdoa}{
short=PDOA,
long= phase-difference-of-arrival,
}
\DeclareAcronym{prs}{
short=PRS,
long= positioning reference signals,
}
\DeclareAcronym{peb}{
short=PEB,
long= position error bound,
}
\DeclareAcronym{speb}{
short=SPEB,
long= squared position error bound,
}
\DeclareAcronym{rnn}{
short=RNN,
long= recurrent neural network,
}
\DeclareAcronym{rl}{
short=RL,
long= reinforcement learning,
}
\DeclareAcronym{rfc}{
short=RFC,
long= radio-frequency chain,
}
\DeclareAcronym{rf}{
short=RF,
long= radio frequency,
}
\DeclareAcronym{rfid}{
short=RFID,
long= radio frequency identification,
}
\DeclareAcronym{ris}{
short=RIS,
long= reconfigurable intelligent surface,
}
\DeclareAcronym{rss}{
short=RSS,
long= received signal strength,
}
\DeclareAcronym{rtt}{
short=RTT,
long= round-trip time,
}
\DeclareAcronym{sm}{
short=SM,
long= standard model,
}
\DeclareAcronym{sige}{
short=SiGe,
long= silicon-germanium,
}
\DeclareAcronym{spp}{
short=SPP,
long= surface plasmon polariton,
}
\DeclareAcronym{sa}{
short=SA,
long= subarray,
}
\DeclareAcronym{sota}{
short=SOTA,
long= state-of-the-art,
}
\DeclareAcronym{swm}{
short=SWM,
long= spherical wave model,
}
\DeclareAcronym{slam}{
short=SLAM,
long= simultaneous localization and mapping,
}
\DeclareAcronym{tm}{
short=TM,
long= true model,
}
\DeclareAcronym{toa}{
short=TOA,
long= time-of-arrival,
}
\DeclareAcronym{tof}{
short=TOF,
long= time-of-flight,
}
\DeclareAcronym{tdoa}{
short=TDOA,
long= time-difference-of-arrival,
}
\DeclareAcronym{thz}{
short=THz,
long= Terahertz,
}
\DeclareAcronym{ue}{
short=UE,
long= user equipment,
}
\DeclareAcronym{ummimo}{
short=UM-MIMO,
long= ultra-massive multi-input-multi-output,
}
\DeclareAcronym{vlp}{
short=VLP,
long= visible light positioning,
}
\DeclareAcronym{veb}{
short=VEB,
long= velocity error bound,
}
\DeclareAcronym{vlc}{
short=VLC,
long= visible light communication,
}
\DeclareAcronym{ula}{
short=ULA,
long= uniform linear array,
}
\DeclareAcronym{uav}{
short=UAV,
long= unmanned aerial vehicle,
}
\DeclareAcronym{upa}{
short=UPA,
long= uniform planar array,
}
\DeclareAcronym{wlan}{
short=WLAN,
long= wireless local area network,
}
\DeclareAcronym{gcs}{
short=GCS,
long= global coordinate system,
}
\DeclareAcronym{lcs}{
short=LCS,
long= local coordinate system,
}
\DeclareAcronym{awgn}{
short=AWGN,
long= additive white Gaussian noise,
}
\DeclareAcronym{iid}{
short=i.i.d.,
long= independent and identically distributed,
}
\DeclareAcronym{snr}{
short=SNR,
long= signal-to-noise ratio,
}
\DeclareAcronym{csir}{
short=CSIR,
long= channel state information at the receiver,
}
\DeclareAcronym{cdit}{
short=CDIT,
long= channel distribution information at the transmitter,
}
\DeclareAcronym{tbps}{
short=Tbps,
long= Terabit-per-second,
}
\DeclareAcronym{um-mimo}{
short=UM-MIMO,
long= ultra-massive multiple-input multiple-output,
}
\DeclareAcronym{rmse}{
short=RMSE,
long= root mean square error,
}
\DeclareAcronym{mse}{
short=MSE,
long= mean squared error,
}
\DeclareAcronym{ccdf}{
short=CCDF,
long= complementary cumulative distribution function,
}
\DeclareAcronym{ae}{
short=AE,
long= antenna element,
}
\DeclareAcronym{mrc}{
short=MRC,
long= maximum ratio combining,
}
\DeclareAcronym{egc}{
short=EGC,
long= equal gain combining,
}
\DeclareAcronym{dft}{
short=DFT,
long= discrete Fourier transform,
}
\DeclareAcronym{kld}{
short=KLD,
long= Kullback–Leibler divergence,
}











==> RIS Geometry Mismatch/figures/MCRB_vs_P.tex <==
\begin{tikzpicture}

\begin{axis}[%
width=2.75in,
height=1.4in,
at={(0in,0in)},
scale only axis,
xmin=-10,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={Transmitted power $P$ [dBm]},
ymode=log,
ymin=3e-03,
ymax=10,
ylabel style={font=\color{white!15!black}},
ylabel={RMSE [$\unit[]{m}$]},
yminorticks=true,
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0,1)}, font=\scriptsize, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=blue, mark=x, mark size=3.3pt,mark options={solid, blue},line width=1pt]
  table[row sep=crcr]{%
  -10	0.889128502738626\\
  -5	0.482304265897224\\
  0	0.267935878248287\\
  5	0.151211587665345\\
  10	0.087441309573895\\
  15	0.0534627937329172\\
  20	0.0366025775267849\\
  25	0.0292287293399754\\
  30	0.0264058137774717\\
  35	0.0254083832056156\\
  40	0.0250512940124719\\
};
\addlegendentry{ML (pos. mismatch)}

\addplot [color=blue, dashed, mark=square, mark size=3pt,mark options={solid, blue},line width=1pt]
  table[row sep=crcr]{%
  -10	0.846403217503069\\
  -5	0.476410094926132\\
  0	0.268690565089602\\
  5	0.152484192639236\\
  10	0.0881716134558079\\
  15	0.0536648331087028\\
  20	0.0364992428807203\\
  25	0.0290303775376409\\
  30	0.0262295798717661\\
  35	0.025279392182549\\
  40	0.0249713930966303\\
};
\addlegendentry{LB (pos. mismatch)}

\addplot [color=blue, dashed,line width=1pt]
  table[row sep=crcr]{%
  -10	0.0248275677523335\\
  -5	0.0248276537125904\\
  0	0.0248276537125632\\
  5	0.0248276537125525\\
  10	0.0248276587133737\\
  15	0.0248276587133554\\
  20	0.0248276590197878\\
  25	0.0248276590187157\\
  30	0.0248276590197902\\
  35	0.0248276590188475\\
  40	0.0248276590197731\\
};
\addlegendentry{Bias (pos. mismatch)}


\end{axis}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{axis}[%
  width=2.75in,
  height=1.4in,
  at={(0in,0in)},
  scale only axis,
  xmin=-10,
  xmax=40,
  xtick={\empty},
  ymode=log,
  ymin=3e-03,
  ymax=10,
  ytick={\empty},
  legend style={at={(1,1)}, font=\scriptsize, anchor=north east, legend cell align=left, align=left, draw=white!15!black, fill opacity=1}
  ]
  
  \addplot [color=red, mark=+, mark size=3.6pt,mark options={solid, red},line width=1pt]
    table[row sep=crcr]{%
    -10	0.945701796948886\\
    -5	0.537223830011796\\
    0	0.335916380883954\\
    5	0.24229257520225\\
    10	0.20368877021528\\
    15	0.189382237923837\\
    20	0.184299099982199\\
    25	0.182484961873893\\
    30	0.181830709725284\\
    35	0.181542339667633\\
    40	0.181439992687649\\
  };
  \addlegendentry{ML (ori. mismatch)}
  
  \addplot [color=red, dashed, mark=o, mark size=3.6pt,mark options={solid, red},line width=1pt]
    table[row sep=crcr]{%
    -10	0.886436425248452\\
    -5	0.520509349217151\\
    0	0.328821123219376\\
    5	0.237990224365415\\
    10	0.200894702764253\\
    15	0.18764403315994\\
    20	0.183254513314695\\
    25	0.181844375287026\\
    30	0.181396169117403\\
    35	0.181254203223822\\
    40	0.181209286519745\\
  };
  \addlegendentry{LB (ori. mismatch)}
  
  \addplot [color=red, dashed,line width=1pt]
    table[row sep=crcr]{%
    -10	0.181188271622172\\
    -5	0.181188509879586\\
    0	0.18118850982267\\
    5	0.18118850982265\\
    10	0.18118850984642\\
    15	0.18118850984635\\
    20	0.18118850984642\\
    25	0.181188509888167\\
    30	0.181188509888129\\
    35	0.18118850988818\\
    40	0.181188509888172\\
  };
  \addlegendentry{Bias (ori. mismatch)}
  
  \addplot [color=black,line width=1pt]
    table[row sep=crcr]{%
    -10	0.841193299768545\\
    -5	0.473037754932775\\
    0	0.266008677973854\\
    5	0.149587672483945\\
    10	0.084119329976739\\
    15	0.0473037754932892\\
    20	0.026600867797375\\
    25	0.0149587672483941\\
    30	0.00841193299768473\\
    35	0.00473037754933004\\
    40	0.00266008677974184\\
  };
  \addlegendentry{Mismatch-free PEB}
  
  \end{axis}


\end{tikzpicture}%

==> RIS Geometry Mismatch/figures/MCRB_vs_sigma2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
  \begin{axis}[%
    width=2.75in,
    height=0.6in,
    at={(0in,0in)},
  scale only axis,
  xmin=0.09,
  xmax=0.61,
  xlabel style={font=\color{white!15!black}},
  xlabel={$\unit[\sigma_\mathrm{o}]{[{deg}]}$},
  ymode=log,
  ymin=0.05,
  ymax=1,
  yminorticks=true,
  ylabel style={font=\color{white!15!black}},
  ylabel={RMSE [$\unit[]{m}$]},
  axis background/.style={fill=white},
  xmajorgrids,
  ymajorgrids,
  yminorgrids,
  legend style={at={(0,1)}, font=\scriptsize, anchor=north west,legend cell align=left, align=left, draw=white!15!black}
  ]
  
  \addplot [color=blue, line width=1.0pt, mark=o, mark options={solid, blue}]
   plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=4.0pt, rotate=90}]
   table[row sep=crcr, y error plus index=2, y error minus index=3]{%
   0.1	0.0929907680490119	0.0292649245536898	0.00888393944481572\\
   0.2	0.113974157352882	0.082421703522655	0.029827416445583\\
   0.3	0.140753854905995	0.140167486679762	0.0565177753158361\\
   0.4	0.170574123207005	0.199258077500105	0.0862022961009108\\
   0.5	0.201909075310515	0.25822668200503	0.117358121336454\\
   0.6	0.234634959092299	0.321310957919717	0.14986452459521\\
  };
  \addlegendentry{LB (ori. mismatch)}
  
  \addplot [color=red, dashed, line width=1.5pt]
    table[row sep=crcr]{%
    0.1	0.084119329976739\\
    0.2	0.084119329976739\\
    0.3	0.084119329976739\\
    0.4	0.084119329976739\\
    0.5	0.084119329976739\\
    0.6	0.084119329976739\\
  };
  \addlegendentry{Mismatch-free PEB}
  
  \end{axis}


  \begin{axis}[%
    width=2.75in,
    height=0.6in,
    at={(0in,0in)},
  scale only axis,
  xmin=0.09,
  xmax=0.61,
  ymode=log,
  ymin=0.05,
  ymax=1,
  yminorticks=false,
  xtick={\empty},
  ytick={\empty},
  legend style={at={(0,1)}, font=\scriptsize, anchor=north west,legend cell align=left, align=left, draw=white!15!black}
  ]
  
  \addplot [color=blue, line width=1.0pt, mark=o, mark options={solid, blue}, forget plot]
   plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=4.0pt, rotate=90}]
   table[row sep=crcr, y error plus index=2, y error minus index=3]{%
   0.1	0.0929907680490119	0.0292649245536898	0.00888393944481572\\
   0.2	0.113974157352882	0.082421703522655	0.029827416445583\\
   0.3	0.140753854905995	0.140167486679762	0.0565177753158361\\
   0.4	0.170574123207005	0.199258077500105	0.0862022961009108\\
   0.5	0.201909075310515	0.25822668200503	0.117358121336454\\
   0.6	0.234634959092299	0.321310957919717	0.14986452459521\\
  };
  
  \addplot [color=red, dashed, line width=1.5pt, forget plot]
    table[row sep=crcr]{%
    0.1	0.084119329976739\\
    0.2	0.084119329976739\\
    0.3	0.084119329976739\\
    0.4	0.084119329976739\\
    0.5	0.084119329976739\\
    0.6	0.084119329976739\\
  };
  
  \end{axis}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\begin{axis}[%
  width=2.75in,
  height=0.6in,
  at={(0in,1.1in)},
scale only axis,
xlabel style={font=\color{white!15!black}},
xlabel={$\unit[\sigma_\mathrm{p}]{[m]}$},
xmin=0.009,
xmax=0.061,
ymode=log,
ymin=0.05,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={RMSE [$\unit[]{m}$]},
xtick={0.01,0.02,0.03,0.04,0.05,0.06},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0,1)}, font=\scriptsize, anchor=north west,legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=blue, line width=1.0pt, mark=o, mark options={solid, blue}]
 plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=4.0pt, rotate=90}]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
 0.01	0.0932726753428712	0.0445579049873599	0.00893012007313974\\
 0.02	0.114329550360036	0.120476966430145	0.0293398761819626\\
 0.03	0.141018914976076	0.200869843716523	0.0549677946469987\\
 0.04	0.1707647646209	0.282896784223409	0.0832529491994101\\
 0.05	0.202277460076893	0.366531236581574	0.112925281843744\\
 0.06	0.234928442429327	0.4519889736101	0.143379130353293\\
};
\addlegendentry{LB (pos. mismatch)}

\addplot [color=red, dashed, line width=1.5pt]
  table[row sep=crcr]{%
  0.01	0.084119329976739\\
  0.02	0.084119329976739\\
  0.03	0.084119329976739\\
  0.04	0.084119329976739\\
  0.05	0.084119329976739\\
  0.06	0.084119329976739\\
};
\addlegendentry{Mismatch-free PEB}

\end{axis}

\begin{axis}[%
  width=2.75in,
  height=0.6in,
  at={(0in,1.1in)},
scale only axis,
xmin=0.009,
xmax=0.061,
ymode=log,
ymin=0.05,
ymax=1,
yminorticks=false,
xtick={\empty},
ytick={\empty},
xticklabels = {\empty},
yticklabels = {\empty},
legend style={at={(0,1)}, font=\scriptsize, anchor=north west,legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=blue, line width=1.0pt, mark=o, mark options={solid, blue}, forget plot]
 plot [error bars/.cd, y dir=both, y explicit, error bar style={line width=1.0pt}, error mark options={line width=1.0pt, mark size=4.0pt, rotate=90}]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
 0.01	0.0932726753428712	0.0445579049873599	0.00893012007313974\\
 0.02	0.114329550360036	0.120476966430145	0.0293398761819626\\
 0.03	0.141018914976076	0.200869843716523	0.0549677946469987\\
 0.04	0.1707647646209	0.282896784223409	0.0832529491994101\\
 0.05	0.202277460076893	0.366531236581574	0.112925281843744\\
 0.06	0.234928442429327	0.4519889736101	0.143379130353293\\
};

\addplot [color=red, dashed, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
  0.01	0.084119329976739\\
  0.02	0.084119329976739\\
  0.03	0.084119329976739\\
  0.04	0.084119329976739\\
  0.05	0.084119329976739\\
  0.06	0.084119329976739\\
};

\end{axis}






\end{tikzpicture}%
